Mean Payoff Optimization for Systems of Periodic Service and Maintenance

Consider oriented graph nodes requiring periodic visits by a service agent. The agent moves among the nodes and receives a payoff for each completed service task, depending on the time elapsed since the previous visit to a node. We consider the problem of finding a suitable schedule for the agent to maximize its long-run average payoff per time unit. We show that the problem of constructing an $\varepsilon$-optimal schedule is PSPACE-hard for every fixed $\varepsilon \geq 0$, and that there exists an optimal periodic schedule of exponential length. We propose randomized finite-memory (RFM) schedules as a compact description of the agent's strategies and design an efficient algorithm for constructing RFM schedules. Furthermore, we construct deterministic periodic schedules by sampling from RFM schedules.

==> dcolumn.tex <==
\makeatletter
\def\DC@#1#2#3{%
  \uccode`\~=`#1\relax
  \m@th
  \afterassignment\DC@x\count@#3\relax{#1}{#2}}
\def\DC@x#1\relax#2#3{%
  \ifnum\z@>\count@
    \expandafter\DC@centre
  \else
    \expandafter\DC@right
  \fi
  {#2}{#3}{#1}}
\def\DC@centre#1#2#3{%
  \let\DC@end\DC@endcentre
  \uppercase{\def~}{\egroup\setbox\tw@=\hbox\bgroup{#2}}%
  \setbox\tw@=\hbox{{\phantom{{#2}}}}%
  \setbox\z@=\hbox\bgroup\catcode`#1=13 }
\def\DC@endcentre{\egroup
    \ifdim \wd\z@>\wd\tw@
      \setbox\tw@=\hbox to\wd\z@{\unhbox\tw@\hfill}%
    \else
      \setbox\z@=\hbox to\wd\tw@{\hfill\unhbox\z@}\fi
    \box\z@\box\tw@}
\def\DC@right#1#2#3{%
  \ifx\relax#3\relax
    \hfill
    \let\DC@rl\bgroup
  \else
    \edef\DC@rl{to\the\count@\dimen@ii\bgroup\hss\hfill}%
    \count@\@gobble#3\relax
  \fi
  \let\DC@end\DC@endright
  \uppercase{\def~}{\egroup\setbox\tw@\hbox to\dimen@\bgroup{#2}}%
   \setbox\z@\hbox{1}\dimen@ii\wd\z@
   \dimen@\count@\dimen@ii
   \setbox\z@\hbox{{#2}}\advance\dimen@\wd\z@
   \setbox\tw@\hbox to\dimen@{}%
   \setbox\z@\hbox\DC@rl\catcode`#1=13 }
\def\DC@endright{\hfil\egroup\box\z@\box\tw@}
\newcolumntype{D}[3]{>{\DC@{#1}{#2}{#3}}c<{\DC@end}}
\makeatother
\endinput

